SPARC: Single-Pass Scaling for Motion Forecasting with Conformal Bayesian Last Layers

Human motion forecasters are increasingly accurate and fast, but reliable deployment requires uncertainty estimates that are structured, calibrated, and efficient. Bayesian and ensemble-based uncertainty estimates often require repeated stochastic inference [15, 26], while conformal calibration alone does not provide an epistemic signal or preserve trajectory covariance structure [14, 50]. We introduce SPARC (Single-Pass Adaptive Risk Calibration), a Bayesian-conformal uncertainty layer for motion forecasting. A deterministic MLP backbone predicts the future mean, and a conjugate Bayesian last layer converts time-domain feature leverage into an analytic horizon-wise epistemic scale $\kappa_t(x)$. This scale inflates a graph-temporal Gaussian covariance without changing its correlation structure, and split conformal calibration produces 95% marginal prediction tubes with finite-sample validity under exchangeability. The key interface is the structured factorization $\kappa_t(x)\Sigma_{\mathrm{str},t}(x)$, which injects feature-space epistemic uncertainty into trajectory densities without Monte Carlo sampling. Across nine dataset-protocol blocks and deterministic, multimodal, and calibration baselines, SPARC ranks first on NLL and on the combined MPJPE+NLL criterion while retaining competitive point accuracy and efficient calibrated tubes. Ranking windows by $\kappa$ separates high-error cases, making the scale usable as a lightweight risk monitor.

==> tables/amass_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.000347,1.002331) & 200 & 0.964 & 0.128 & 0.914 & 0.078 \\
20--40\% [1.002331,1.003692) & 207 & 0.945 & 0.138 & 0.908 & 0.101 \\
40--60\% [1.003692,1.005284) & 203 & 0.920 & 0.141 & 0.905 & 0.125 \\
60--80\% [1.005284,1.008165) & 209 & 0.881 & 0.143 & 0.889 & 0.149 \\
80--100\% [1.008165,1.031798) & 205 & 0.804 & 0.144 & 0.900 & 0.234 \\
\midrule
All & 1024 & 0.902 & 0.139 & 0.903 & 0.138 \\
\bottomrule
\end{tabular}
\caption{AMASS: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:amass_kappa_mondrian}
\end{table}


==> tables/amass_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.902 & -2.105 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.924 & -1.955 \\
\bottomrule
\end{tabular}
\caption{AMASS: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:amass_traj_set}
\end{table}


==> tables/andy_oneperson_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.003514,1.003549) & 224 & 0.998 & 0.068 & 0.892 & 0.008 \\
20--40\% [1.003549,1.003646) & 224 & 0.992 & 0.068 & 0.897 & 0.014 \\
40--60\% [1.003646,1.009277) & 156 & 0.949 & 0.068 & 0.882 & 0.036 \\
60--80\% [1.009277,1.220523) & 209 & 0.781 & 0.075 & 0.895 & 0.135 \\
80--100\% [1.220523,1.713087) & 211 & 0.772 & 0.101 & 0.912 & 0.177 \\
\midrule
All & 1024 & 0.898 & 0.076 & 0.896 & 0.074 \\
\bottomrule
\end{tabular}
\caption{AnDy-onePerson: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:andy_kappa_mondrian}
\end{table}


==> tables/andy_oneperson_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.898 & -2.815 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.922 & -3.007 \\
\bottomrule
\end{tabular}
\caption{AnDy-onePerson: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:andy_traj_set}
\end{table}


==> tables/baselines_bestk_overview_all_datasets.tex <==
\begin{table}[t]
\centering
\caption{Baseline results overview (best-of-K MPJPE, H=25). All entries are external baselines; our proposed models are intentionally omitted. Missing entries (``--'') indicate results not yet available under the standard protocol ($\alpha{=}0.1$, seed=304, eval\_calib\_size=512, eval\_size=1024; non-H36M uses $T{=}50$,$H{=}25$). NLL is the Gaussian NLL used in the main benchmark tables. Cov90(CP)/W90(CP) report split-conformal calibrated 90\% marginal tubes (one $q_t$ per horizon; coverage/width averaged over coordinates). Dataset-specific protocol-only baselines (e.g., CHICO-only SeSGCN protocol variants) are omitted.}
\label{tab:baselines_all_bestk}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\providecommand{\missing}{--}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l *{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{AMASS} & \multicolumn{4}{c}{LaFAN1} & \multicolumn{4}{c}{LaFAN1-HF} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} \\
\midrule
\baseline{siMLPe (base)} & 0.0919 & 12.76 & \missing & \missing & 0.4138 & 172.21 & \missing & \missing & 0.4046 & 172.36 & \missing & \missing \\
\baseline{MeanFT (siMLPe fine-tune)} & 0.0588 & 3.04 & \missing & \missing & 0.4138 & 172.20 & \missing & \missing & 0.3093 & 99.80 & \missing & \missing \\
\baseline{AuxTasks (50/50)} & 0.0949 & 12.39 & \missing & \missing & 0.4136 & 171.96 & \missing & \missing & 0.4299 & 184.26 & \missing & \missing \\
\baseline{Symplectic (50/50)} & 0.1424 & 39.70 & \missing & \missing & 1.4504 & 3203.83 & \missing & \missing & 0.4756 & 280.68 & \missing & \missing \\
\baseline{DeFeeNet (50/50)} & 0.0909 & 12.15 & \missing & \missing & 0.5666 & 341.82 & \missing & \missing & 0.3992 & 169.44 & \missing & \missing \\
\baseline{GSPS (50/50)} & 0.0872 & 11.30 & 0.903 & 0.202 & 0.4132 & 171.76 & 0.927 & 1.170 & 0.3737 & 148.57 & 0.900 & 0.927 \\
\baseline{HumanMAC (50/50)} & 0.0722 & 4.34 & \missing & \missing & 0.5564 & 290.09 & \missing & \missing & 0.4477 & 166.64 & \missing & \missing \\
\baseline{SeSGCN (teacher)} & 0.1029 & 9.48 & \missing & \missing & 0.5872 & 314.76 & \missing & \missing & 0.4061 & 138.80 & \missing & \missing \\
\baseline{Deep ensemble} & 0.0869 & 3.27 & 0.902 & 0.190 & 0.4141 & 158.96 & 0.920 & 1.155 & 0.3894 & 80.18 & 0.899 & 0.897 \\
\baseline{Bridge-CQR} & 0.0588 & 0.10 & 0.906 & 0.311 & 0.5358 & 139.07 & 0.899 & 1.541 & 0.3103 & 45.42 & 0.945 & 1.167 \\
\baseline{SkeletonDiffusion (CVPR 2025)} & 0.0947 & 9.03 & 0.900 & 0.221 & 0.5805 & 280.51 & 0.903 & 1.992 & 1.8047 & 3356.76 & 0.914 & 25.800 \\
\baseline{BeLFusion (ICCV 2023)} & 0.0681 & 3.87 & 0.904 & 0.165 & 0.5103 & 251.84 & 0.900 & 1.382 & 0.7068 & 524.85 & 0.908 & 2.211 \\
\baseline{TransFusion (RA-L 2024)} & 0.0737 & 3.81 & 0.902 & 0.148 & 0.6342 & 324.41 & 0.898 & 1.487 & 1.0187 & 1240.56 & 0.913 & 2.475 \\
\baseline{CoMusion (ECCV 2024)} & 0.0536 & 1.40 & 0.906 & 0.125 & 0.4754 & 217.70 & 0.900 & 1.184 & 0.3201 & 93.39 & 0.902 & 0.928 \\
\baseline{SPARD (AAAI 2026)} & 0.0554 & 1.51 & 0.906 & 0.128 & 0.5197 & 292.29 & 0.903 & 1.303 & 0.3432 & 105.81 & 0.907 & 0.851 \\
\baseline{MotionMap (CVPR 2025)} & 0.1283 & 16.42 & 0.898 & 0.404 & 0.6626 & 351.70 & 0.899 & 1.568 & 0.7384 & 470.72 & 0.907 & 3.408 \\
\baseline{SLD-HMP (ECCV 2024)} & 0.1487 & 22.41 & 0.901 & 0.224 & 0.7521 & 491.40 & 0.904 & 1.441 & 0.7077 & 399.22 & 0.901 & 1.035 \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CMU-MoCap} & \multicolumn{4}{c}{Human3.6M} & \multicolumn{4}{c}{3DPW} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE$_{\text{bestK}}\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} \\
\midrule
\baseline{siMLPe (base)} & 2.4528 & 7350.97 & \missing & \missing & 0.1012 & 12.84 & \missing & \missing & 0.0686 & 4.75 & \missing & \missing \\
\baseline{MeanFT (siMLPe fine-tune)} & 2.4521 & 7350.10 & \missing & \missing & 0.0720 & 5.24 & \missing & \missing & 0.0572 & 1.71 & \missing & \missing \\
\baseline{AuxTasks (50/50)} & 2.4588 & 7380.92 & \missing & \missing & 0.0877 & 10.69 & \missing & \missing & 0.0745 & 5.27 & \missing & \missing \\
\baseline{Symplectic (50/50)} & 4.1748 & 24392.45 & \missing & \missing & 0.1070 & 13.08 & \missing & \missing & 0.1042 & 20.62 & \missing & \missing \\
\baseline{DeFeeNet (50/50)} & 2.6316 & 8633.05 & \missing & \missing & 0.0981 & 12.31 & \missing & \missing & 0.0701 & 4.99 & \missing & \missing \\
\baseline{GSPS (50/50)} & 2.4246 & 7292.37 & 0.910 & 7.894 & 0.0922 & 11.31 & 0.917 & 0.270 & 0.0654 & 4.00 & 0.899 & 0.150 \\
\baseline{HumanMAC (50/50)} & 4.8433 & 21062.22 & \missing & \missing & 0.0982 & 7.83 & \missing & \missing & 0.0707 & 2.68 & \missing & \missing \\
\baseline{SeSGCN (teacher)} & 4.9092 & 20996.24 & \missing & \missing & 0.1119 & 9.85 & \missing & \missing & 0.0952 & 5.32 & \missing & \missing \\
\baseline{Deep ensemble} & 2.4414 & 1108.28 & 0.917 & 8.693 & 0.0717 & 1.72 & 0.891 & 0.153 & 0.0577 & 0.79 & 0.897 & 0.131 \\
\baseline{Bridge-CQR} & 2.5631 & 3830.90 & 0.920 & 6.974 & 0.0843 & 2.25 & 0.924 & 0.493 & 0.0581 & -0.50 & 0.917 & 0.403 \\
\baseline{SkeletonDiffusion (CVPR 2025)} & 7.9889 & 49452.99 & 0.903 & 251.141 & 0.1210 & 13.55 & 0.897 & 0.284 & 0.0806 & 4.91 & 0.896 & 0.173 \\
\baseline{BeLFusion (ICCV 2023)} & 3.5539 & 12250.77 & 0.905 & 10.220 & 0.0936 & 6.30 & 0.897 & 0.234 & 0.0658 & 2.08 & 0.896 & 0.154 \\
\baseline{TransFusion (RA-L 2024)} & 7.6277 & 44784.36 & 0.903 & 21.434 & 0.1002 & 7.14 & 0.897 & 0.223 & 0.0735 & 2.75 & 0.892 & 0.146 \\
\baseline{CoMusion (ECCV 2024)} & 8.6798 & 54190.65 & 0.905 & 21.069 & 0.0816 & 4.70 & 0.895 & 0.214 & 0.0604 & 1.20 & 0.895 & 0.135 \\
\baseline{SPARD (AAAI 2026)} & 5.3451 & 25772.76 & 0.906 & 20.408 & 0.0801 & 4.26 & 0.891 & 0.186 & 0.0610 & 1.26 & 0.895 & 0.136 \\
\baseline{MotionMap (CVPR 2025)} & 4.8192 & 21490.67 & 0.902 & 13.803 & 0.1873 & 29.09 & 0.897 & 0.547 & 0.1140 & 9.58 & 0.897 & 0.382 \\
\baseline{SLD-HMP (ECCV 2024)} & 4.2042 & 16849.58 & 0.901 & 8.420 & 0.1787 & 26.16 & 0.894 & 0.263 & 0.1373 & 15.84 & 0.899 & 0.173 \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CHICO} & \multicolumn{4}{c}{HA4M} & \multicolumn{4}{c}{AnDy-onePerson} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE@10/25f$_{\text{bestK}}$ (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f$_{\text{bestK}}$ (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f$_{\text{bestK}}$ (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov90{\tiny(CP)}} & {W90{\tiny(CP)}$\downarrow$} \\
\midrule
\baseline{siMLPe (base)} & 43.2 / 75.2 & 0.66 & \missing & \missing & 34.6 / 67.1 & -0.63 & \missing & \missing & 4.7 / 6.8 & -3.13 & \missing & \missing \\
\baseline{MeanFT (siMLPe fine-tune)} & 42.7 / 64.8 & -0.35 & \missing & \missing & 34.6 / 67.2 & -0.63 & \missing & \missing & 4.7 / 6.7 & -3.13 & \missing & \missing \\
\baseline{AuxTasks (50/50)} & 44.6 / 77.7 & 0.88 & \missing & \missing & 34.7 / 67.1 & -0.63 & \missing & \missing & 16.4 / 9.6 & -3.06 & \missing & \missing \\
\baseline{Symplectic (50/50)} & 46.6 / 91.2 & 0.77 & \missing & \missing & 79.5 / 364.9 & 24.42 & \missing & \missing & 30.2 / 105.5 & 2.62 & \missing & \missing \\
\baseline{DeFeeNet (50/50)} & 42.7 / 75.2 & 0.69 & \missing & \missing & 93.5 / 77.2 & 3.11 & \missing & \missing & 26.1 / 72.6 & 1.75 & \missing & \missing \\
\baseline{GSPS (50/50)} & 42.1 / 77.8 & 0.57 & 0.895 & 0.118 & 48.1 / 54.4 & -0.98 & 0.872 & 0.097 & 5.5 / 6.6 & -3.12 & 1.000 & 0.155 \\
\baseline{HumanMAC (50/50)} & 52.0 / 70.7 & 0.27 & \missing & \missing & 189.5 / 196.7 & 35.25 & \missing & \missing & 55.7 / 80.0 & 1.98 & \missing & \missing \\
\baseline{SeSGCN (teacher)} & 66.2 / 77.7 & 1.43 & \missing & \missing & 150.9 / 171.5 & 21.59 & \missing & \missing & 55.7 / 81.3 & 2.05 & \missing & \missing \\
\baseline{Deep ensemble} & 41.3 / 78.3 & -0.21 & 0.894 & 0.116 & 35.8 / 67.4 & -0.94 & 0.891 & 0.097 & 5.7 / 6.8 & -3.09 & 0.999 & 0.156 \\
\baseline{Bridge-CQR} & 42.7 / 65.0 & -1.46 & 0.910 & 0.434 & 42.0 / 76.7 & -1.73 & 0.986 & 0.533 & 27.0 / 55.0 & -1.46 & 0.932 & 0.894 \\
\baseline{SkeletonDiffusion (CVPR 2025)} & 56.8 / 75.6 & 1.41 & 0.902 & 0.145 & 179.9 / 159.8 & 26.99 & 0.908 & 0.563 & 62.4 / 88.2 & 4.60 & 0.896 & 0.156 \\
\baseline{BeLFusion (ICCV 2023)} & 41.0 / 55.3 & -1.04 & 0.898 & 0.113 & 134.5 / 111.8 & 8.34 & 0.898 & 0.271 & 33.9 / 55.0 & -0.15 & 0.899 & 0.093 \\
\baseline{TransFusion (RA-L 2024)} & 43.3 / 57.4 & -0.76 & 0.897 & 0.104 & 120.2 / 118.9 & 10.26 & 0.855 & 0.242 & 42.7 / 62.5 & 0.05 & 0.899 & 0.112 \\
\baseline{CoMusion (ECCV 2024)} & 37.8 / 50.9 & -1.28 & 0.899 & 0.099 & 153.2 / 164.3 & 22.76 & 0.900 & 0.335 & 28.2 / 46.7 & -1.31 & 0.899 & 0.076 \\
\baseline{SPARD (AAAI 2026)} & 37.4 / 49.4 & -1.40 & 0.900 & 0.099 & 147.8 / 169.5 & 21.26 & 0.895 & 0.345 & 27.9 / 47.9 & -1.40 & 0.900 & 0.076 \\
\baseline{MotionMap (CVPR 2025)} & 76.8 / 81.4 & 3.15 & 0.904 & 0.354 & 250.2 / 226.7 & 52.42 & 0.928 & 0.352 & 128.1 / 137.2 & 15.52 & 0.899 & 0.391 \\
\baseline{SLD-HMP (ECCV 2024)} & 58.0 / 73.5 & 4.19 & 0.895 & 0.122 & 69.7 / 61.9 & 7.37 & 0.890 & 0.127 & 68.0 / 85.6 & 7.92 & 0.898 & 0.119 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/chico_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.001235,1.020121) & 194 & 0.954 & 0.091 & 0.900 & 0.058 \\
20--40\% [1.020121,1.046963) & 188 & 0.906 & 0.096 & 0.899 & 0.095 \\
40--60\% [1.046963,1.076667) & 203 & 0.886 & 0.101 & 0.896 & 0.107 \\
60--80\% [1.076667,1.116312) & 216 & 0.872 & 0.107 & 0.887 & 0.113 \\
80--100\% [1.116312,1.470618) & 223 & 0.870 & 0.117 & 0.909 & 0.138 \\
\midrule
All & 1024 & 0.896 & 0.103 & 0.898 & 0.103 \\
\bottomrule
\end{tabular}
\caption{CHICO: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:chico_kappa_mondrian}
\end{table}


==> tables/chico_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.896 & -2.387 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.900 & -1.926 \\
\bottomrule
\end{tabular}
\caption{CHICO: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:chico_traj_set}
\end{table}


==> tables/cmu_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [3.934778,5.150264) & 65 & 0.885 & 5.936 & 0.899 & 6.333 \\
20--40\% [5.150264,5.501943) & 54 & 0.853 & 6.557 & 0.900 & 8.034 \\
40--60\% [5.501943,6.046422) & 87 & 0.889 & 7.030 & 0.913 & 7.832 \\
60--80\% [6.046422,6.412234) & 58 & 0.943 & 7.549 & 0.905 & 5.973 \\
80--100\% [6.412234,6.989321) & 56 & 0.942 & 7.833 & 0.900 & 6.310 \\
\midrule
All & 320 & 0.906 & 7.020 & 0.908 & 6.980 \\
\bottomrule
\end{tabular}
\caption{CMU-MoCap: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=320), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:cmu_kappa_mondrian}
\end{table}


==> tables/cmu_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.906 & 1.785 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.906 & 2.309 \\
\bottomrule
\end{tabular}
\caption{CMU-MoCap: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=320$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:cmu_traj_set}
\end{table}


==> tables/dependence_sensitivity_densityset.tex <==
% Auto-generated by scripts/paper/eval_dependence_sensitivity_nonoverlap.py
\begin{table}[t]
  \centering
  \caption{Dependence sensitivity of density-set CP (target 90\%). We compare default (potentially overlapping) windows to non-overlapping windows (stride $T{+}H$). Reported values are trajectory-level coverage and mean log-volume per dimension.}
  \label{tab:dependence_sensitivity}
  \scriptsize
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.10}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}llrrrr@{}}
    \toprule
    Dataset & Windowing & $n_{\mathrm{cal}}$ & $n_{\mathrm{eval}}$ & Cov90(Set) & logV/dim \\
    \midrule
    Human3.6M & overlap & 322 & 322 & 0.913 & -0.9101 \\
    Human3.6M & non-overlap & 322 & 322 & 0.885 & -0.9190 \\
    CHICO & overlap & 415 & 416 & 0.925 & -1.4298 \\
    CHICO & non-overlap & 415 & 416 & 0.904 & -1.4349 \\
    3DPW & overlap & 259 & 260 & 0.912 & -2.2928 \\
    3DPW & non-overlap & 259 & 260 & 0.904 & -2.2140 \\
    AnDy-onePerson & overlap & 512 & 1024 & 0.882 & -1.2455 \\
    AnDy-onePerson & non-overlap & 512 & 1024 & 0.880 & -1.2564 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/h36m_conjbayes_baselines.tex <==
\setlength{\LTcapwidth}{\linewidth}
\setlength{\LTleft}{\fill}
\setlength{\LTright}{\fill}
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.10}
\begin{longtable}{@{}p{0.48\linewidth}rrrr@{}}
\caption{Human3.6M (H=25; seed=304, $n_{\mathrm{cal}}{=}512$, $n_{\mathrm{eval}}{=}1024$, $\alpha{=}0.05$): common baselines vs.\ SPARC. Cov95(\cp)/W95(\cp) are split-conformal calibrated 95\% marginal tubes when available; deterministic methods do not output $\hat\sigma_{t,c}(x)$ and thus do not report \cp tube metrics.}\label{tab:h36m_baselines_main}\\
\toprule
Model & MPJPE/FDE$\downarrow$ & NLL$\downarrow$ & Cov95(\cp) & W95(\cp)$\downarrow$ \\
\midrule
\endfirsthead
\caption[]{Human3.6M (H=25; seed=304, $n_{\mathrm{cal}}{=}512$, $n_{\mathrm{eval}}{=}1024$, $\alpha{=}0.05$): common baselines vs.\ SPARC. Cov95(\cp)/W95(\cp) are split-conformal calibrated 95\% marginal tubes when available; deterministic methods do not output $\hat\sigma_{t,c}(x)$ and thus do not report \cp tube metrics. (continued)}\\
\toprule
Model & MPJPE/FDE$\downarrow$ & NLL$\downarrow$ & Cov95(\cp) & W95(\cp)$\downarrow$ \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{\footnotesize Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
siMLPe (base) & 0.1012 / 0.1535 & 12.84 & -- & -- \\
MeanFT (siMLPe fine-tune) & \textbf{0.0720} & 5.24 & -- & -- \\
AuxTasks (50/50) & 0.0999 & 12.63 & -- & -- \\
Symplectic (50/50) & 0.1070 / 0.2151 & 13.08 & -- & -- \\
DeFeeNet (50/50) & 0.0981 & 12.31 & -- & -- \\
GSPS (50/50) & 0.0960 / 0.1540 & 10.96 & 0.945 & 0.313 \\
HumanMAC (50/50) & 0.0982 & 7.83 & -- & -- \\
SeSGCN (teacher) & 0.1119 / 0.1505 & 9.85 & -- & -- \\
Deep ensemble & 0.0971 / 0.1515 & 9.12 & 0.946 & 0.337 \\
Bridge-CQR & \underline{0.0721 / 0.1189} & \underline{1.13} & 0.995 & 1.238 \\
SkeletonDiffusion & 0.1242 / 0.1662 & 13.58 & 0.947 & 0.406 \\
BeLFusion & 0.1055 / 0.1512 & 6.22 & \underline{0.948} & 0.316 \\
TransFusion & 0.1060 / 0.1449 & 7.18 & \underline{0.948} & 0.295 \\
CoMusion & 0.0944 / 0.1409 & 4.49 & 0.945 & 0.287 \\
SPARD & 0.0928 / 0.1364 & 4.24 & 0.947 & \underline{0.250} \\
MotionMap & 0.2504 / 0.2530 & 29.09 & \textbf{0.951} & 0.718 \\
SLD-HMP & 0.1170 / 0.1620 & 26.15 & 0.947 & 0.368 \\
\textbf{SPARC$^{\dagger}$} & \underline{0.0721 / 0.1189} & \textbf{-1.66} & 0.946 & \textbf{0.248} \\
\end{longtable}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included). For Cov95(\cp), best/second-best are defined by closeness to the 0.95 target. \quad $^{\dagger}$ (MN-GraphJ, time-coupled $\kappa_t$, shrink).}


==> tables/ha4m_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.109609,1.117494) & 2 & 0.931 & 0.264 & 0.913 & 0.231 \\
20--40\% [1.117494,1.119070) & 0 & -- & -- & -- & -- \\
40--60\% [1.119070,1.121060) & 1 & 0.908 & 0.266 & 0.916 & 0.285 \\
60--80\% [1.121060,1.124058) & 2 & 0.905 & 0.267 & 0.924 & 0.300 \\
80--100\% [1.124058,1.127448) & 8 & 0.891 & 0.267 & 0.911 & 0.304 \\
\midrule
All & 13 & 0.901 & 0.267 & 0.914 & 0.291 \\
\bottomrule
\end{tabular}
\caption{HA4M: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=13), evaluate on disjoint test windows (n=13), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:ha4m_kappa_mondrian}
\end{table}


==> tables/ha4m_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.901 & -1.555 \\
Trajectory ellipsoid (Mahalanobis CP) & 1.000 & -2.382 \\
\bottomrule
\end{tabular}
\caption{HA4M: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=13$, $n_{\mathrm{eval}}=13$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:ha4m_traj_set}
\end{table}


==> tables/lafan1_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.011244,1.118881) & 177 & 0.956 & 1.243 & 0.906 & 0.892 \\
20--40\% [1.118881,1.210466) & 189 & 0.885 & 1.410 & 0.872 & 1.374 \\
40--60\% [1.210466,1.281271) & 217 & 0.906 & 1.522 & 0.913 & 1.580 \\
60--80\% [1.281271,1.355982) & 237 & 0.893 & 1.621 & 0.908 & 1.694 \\
80--100\% [1.355982,1.582801) & 204 & 0.867 & 1.753 & 0.907 & 2.003 \\
\midrule
All & 1024 & 0.900 & 1.522 & 0.902 & 1.534 \\
\bottomrule
\end{tabular}
\caption{LaFAN1: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:lafan1_kappa_mondrian}
\end{table}


==> tables/lafan1_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.900 & 0.207 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.922 & -0.565 \\
\bottomrule
\end{tabular}
\caption{LaFAN1: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:lafan1_traj_set}
\end{table}


==> tables/lafan1_hf_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.000040,1.002010) & 215 & 0.965 & 0.742 & 0.910 & 0.524 \\
20--40\% [1.002010,1.004064) & 219 & 0.925 & 0.747 & 0.891 & 0.629 \\
40--60\% [1.004064,1.005653) & 175 & 0.901 & 0.750 & 0.911 & 0.798 \\
60--80\% [1.005653,1.007545) & 224 & 0.882 & 0.751 & 0.906 & 0.828 \\
80--100\% [1.007545,1.016912) & 191 & 0.834 & 0.757 & 0.894 & 0.941 \\
\midrule
All & 1024 & 0.903 & 0.749 & 0.902 & 0.738 \\
\bottomrule
\end{tabular}
\caption{LaFAN1-HF: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:lafan1_hf_kappa_mondrian}
\end{table}


==> tables/lafan1_hf_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.903 & -0.414 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.887 & 0.211 \\
\bottomrule
\end{tabular}
\caption{LaFAN1-HF: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:lafan1_hf_traj_set}
\end{table}


==> tables/overview_csm_all_datasets.tex <==
\begin{table}[t]
\centering
\caption{Baselines vs. CSM + SPECTRA-CP (Mondrian-pen) across datasets (H=25). Bold marks the best MPJPE/NLL/W95(CP) per dataset among the shown methods (ties included); for Cov95(CP), bold marks the value closest to the 0.95 target. Cov95(CP)/W95(CP) are split-conformal calibrated 95\% marginal tubes (coverage/width averaged over coordinates).}
\label{tab:overview_csm_all}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l *{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{AMASS} & \multicolumn{4}{c}{LaFAN1} & \multicolumn{4}{c}{LaFAN1-HF} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 0.0954 & 13.55 & -- & -- & 0.5453 & 319.27 & -- & -- & 0.4046 & 172.36 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{0.0593} & 3.16 & -- & -- & \underline{0.5358} & 303.33 & -- & -- & \textbf{0.3093} & 99.80 & -- & -- \\
AuxTasks (50/50) & 0.0949 & 12.39 & -- & -- & 0.5827 & 353.83 & -- & -- & 0.4299 & 184.26 & -- & -- \\
Symplectic (50/50) & 0.1424 & 39.70 & -- & -- & 1.4504 & 3203.83 & -- & -- & 0.4756 & 280.68 & -- & -- \\
DeFeeNet (50/50) & 0.0909 & 12.15 & -- & -- & 0.5666 & 341.82 & -- & -- & 0.3992 & 169.44 & -- & -- \\
GSPS (50/50) & 0.0894 & 11.30 & -- & -- & 0.5408 & 282.97 & -- & -- & 0.3833 & 148.57 & -- & -- \\
HumanMAC (50/50) & 0.0722 & 4.34 & -- & -- & 0.5564 & 290.09 & -- & -- & 0.4477 & 166.64 & -- & -- \\
SeSGCN (teacher) & 0.1029 & 9.48 & -- & -- & 0.5872 & 314.76 & -- & -- & 0.4061 & 138.80 & -- & -- \\
Deep ensemble & 0.0869 & 3.27 & -- & -- & 0.5388 & \underline{43.45} & -- & -- & 0.3894 & 80.18 & -- & -- \\
Bridge-CQR & \textbf{0.0588} & \underline{0.10} & -- & -- & \underline{0.5358} & 139.07 & -- & -- & \underline{0.3103} & \underline{45.42} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 0.0971 & 9.02 & \textbf{0.950} & 0.334 & 0.6028 & 280.23 & \underline{0.951} & 4.209 & 1.8071 & 3357.02 & 0.959 & 32.988 \\
BeLFusion (ICCV 2023) & 0.0792 & 3.84 & 0.952 & 0.235 & 0.5618 & 251.70 & 0.952 & 1.894 & 1.0006 & 520.35 & 0.961 & 3.049 \\
TransFusion (RA-L 2024) & 0.0790 & 3.76 & \underline{0.951} & 0.198 & 0.6496 & 324.90 & \textbf{0.950} & 1.847 & 1.4215 & 1222.72 & 0.956 & 3.015 \\
CoMusion (ECCV 2024) & 0.0617 & 1.49 & 0.952 & \textbf{0.174} & \textbf{0.5268} & 219.66 & \underline{0.949} & \textbf{1.590} & 0.3604 & 92.62 & \textbf{0.950} & 1.242 \\
SPARD (AAAI 2026) & 0.0638 & 1.51 & 0.953 & \underline{0.175} & 0.5682 & 292.27 & 0.955 & \underline{1.759} & 0.3677 & 105.70 & 0.954 & \underline{1.078} \\
MotionMap (CVPR 2025) & 0.2038 & 16.42 & \underline{0.949} & 0.536 & 0.7463 & 351.70 & \textbf{0.950} & 2.006 & 1.4691 & 470.72 & 0.953 & 4.645 \\
SLD-HMP (ECCV 2024) & 0.1120 & 22.45 & \underline{0.949} & 0.308 & 0.6091 & 491.37 & 0.955 & 1.936 & 0.4801 & 401.14 & \underline{0.952} & 1.347 \\
\textbf{CSM + SPECTRA-CP (Mondrian-pen)} & 0.0903 & \textbf{-1.71} & \textbf{0.950} & 0.246 & 0.5944 & \textbf{0.99} & 0.955 & 1.861 & 0.3601 & \textbf{-0.33} & \underline{0.948} & \textbf{0.978} \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CMU-MoCap} & \multicolumn{4}{c}{Human3.6M} & \multicolumn{4}{c}{3DPW} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 2.6560 & 8726.23 & -- & -- & 0.1012 & 12.84 & -- & -- & 0.0709 & 5.08 & -- & -- \\
MeanFT (siMLPe fine-tune) & 2.6709 & 8820.46 & -- & -- & \underline{0.0720} & 5.24 & -- & -- & \textbf{0.0572} & 1.71 & -- & -- \\
AuxTasks (50/50) & \textbf{2.5429} & 8292.99 & -- & -- & 0.0999 & 12.63 & -- & -- & 0.0745 & 5.27 & -- & -- \\
Symplectic (50/50) & 6.8024 & 54096.87 & -- & -- & 0.1070 & 13.08 & -- & -- & 0.1042 & 20.62 & -- & -- \\
DeFeeNet (50/50) & 2.6316 & 8633.05 & -- & -- & 0.0981 & 12.31 & -- & -- & 0.0701 & 4.99 & -- & -- \\
GSPS (50/50) & \underline{2.5981} & 8375.43 & -- & -- & 0.0961 & 11.04 & -- & -- & 0.0673 & 4.00 & -- & -- \\
HumanMAC (50/50) & 4.8433 & 21062.22 & -- & -- & 0.0982 & 7.83 & -- & -- & 0.0707 & 2.68 & -- & -- \\
SeSGCN (teacher) & 4.9092 & 20996.24 & -- & -- & 0.1119 & 9.85 & -- & -- & 0.0952 & 5.32 & -- & -- \\
Deep ensemble & 2.6659 & \underline{1786.43} & -- & -- & \textbf{0.0717} & \underline{1.72} & -- & -- & \underline{0.0577} & 0.79 & -- & -- \\
Bridge-CQR & 2.7455 & 4185.33 & -- & -- & 0.0843 & 2.25 & -- & -- & 0.0581 & \underline{-0.50} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 8.0957 & 49441.83 & \textbf{0.950} & 381.727 & 0.1242 & 13.58 & 0.947 & 0.406 & 0.0822 & 4.91 & \underline{0.948} & 0.256 \\
BeLFusion (ICCV 2023) & 3.6186 & 12261.03 & 0.954 & 14.329 & 0.1055 & 6.22 & \underline{0.948} & 0.316 & 0.0771 & 2.13 & \textbf{0.949} & 0.207 \\
TransFusion (RA-L 2024) & 8.0839 & 44901.52 & 0.952 & 25.699 & 0.1060 & 7.18 & \underline{0.948} & 0.295 & 0.0787 & 2.72 & 0.945 & \underline{0.187} \\
CoMusion (ECCV 2024) & 8.6798 & 54190.65 & 0.953 & 24.961 & 0.0944 & 4.49 & 0.945 & \underline{0.287} & 0.0690 & 1.19 & 0.945 & \textbf{0.174} \\
SPARD (AAAI 2026) & 5.5562 & 25823.22 & 0.952 & 37.934 & 0.0928 & 4.24 & 0.947 & \textbf{0.250} & 0.0703 & 1.25 & 0.946 & \textbf{0.174} \\
MotionMap (CVPR 2025) & 5.3103 & 21490.65 & \underline{0.951} & 18.384 & 0.2504 & 29.09 & \textbf{0.951} & 0.718 & 0.1841 & 9.58 & \underline{0.948} & 0.476 \\
SLD-HMP (ECCV 2024) & 2.7547 & 16866.43 & \underline{0.951} & \underline{11.966} & 0.1170 & 26.15 & 0.947 & 0.368 & 0.0846 & 15.79 & \underline{0.948} & 0.235 \\
\textbf{CSM + SPECTRA-CP (Mondrian-pen)} & 2.8169 & \textbf{6.75} & 0.952 & \textbf{10.075} & 0.0972 & \textbf{-1.34} & 0.947 & 0.290 & 0.0773 & \textbf{-1.98} & \textbf{0.949} & 0.217 \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CHICO} & \multicolumn{4}{c}{HA4M} & \multicolumn{4}{c}{AnDy-onePerson} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 43.2 / 75.2 & 0.66 & -- & -- & \underline{46.1 / 57.0} & -1.08 & -- & -- & 28.0 / 70.3 & 2.00 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{42.7 / 64.8} & -0.35 & -- & -- & 53.6 / 57.7 & -1.00 & -- & -- & \underline{27.4 / 55.7} & -0.27 & -- & -- \\
AuxTasks (50/50) & 44.6 / 77.7 & 0.88 & -- & -- & 91.5 / 70.6 & 0.30 & -- & -- & 32.5 / 70.7 & 2.22 & -- & -- \\
Symplectic (50/50) & 46.6 / 91.2 & 0.77 & -- & -- & 79.5 / 364.9 & 24.42 & -- & -- & 30.2 / 105.5 & 2.62 & -- & -- \\
DeFeeNet (50/50) & 42.7 / 75.2 & 0.69 & -- & -- & 93.5 / 77.2 & 3.11 & -- & -- & 26.1 / 72.6 & 1.75 & -- & -- \\
GSPS (50/50) & 42.1 / 77.8 & 0.57 & -- & -- & \textbf{48.1 / 54.4} & -0.98 & -- & -- & 27.5 / 69.3 & 1.47 & -- & -- \\
HumanMAC (50/50) & 52.0 / 70.7 & 0.27 & -- & -- & 189.5 / 196.7 & 35.25 & -- & -- & 55.7 / 80.0 & 1.98 & -- & -- \\
SeSGCN (teacher) & 66.2 / 77.7 & 1.43 & -- & -- & 150.9 / 171.5 & 21.59 & -- & -- & 55.7 / 81.3 & 2.05 & -- & -- \\
Deep ensemble & 41.3 / 78.3 & -0.21 & -- & -- & 121.1 / 67.6 & -0.56 & -- & -- & 25.4 / 69.3 & 0.53 & -- & -- \\
Bridge-CQR & 42.7 / 65.0 & \underline{-1.46} & -- & -- & 42.0 / 76.7 & \textbf{-1.73} & -- & -- & \textbf{27.0 / 55.0} & \underline{-1.46} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 57.7 / 76.8 & 1.41 & 0.952 & 0.214 & 196.7 / 189.9 & 29.06 & 0.958 & 0.778 & 63.3 / 89.7 & 4.60 & \underline{0.949} & 0.265 \\
BeLFusion (ICCV 2023) & 48.4 / 69.7 & -1.04 & \underline{0.949} & 0.150 & 144.4 / 141.6 & 8.99 & \underline{0.951} & 0.344 & 38.7 / 68.5 & -0.14 & \textbf{0.950} & 0.150 \\
TransFusion (RA-L 2024) & 48.6 / 66.4 & -0.81 & \underline{0.949} & 0.133 & 145.5 / 170.8 & 5.43 & 0.944 & 0.296 & 54.7 / 82.1 & 0.07 & \underline{0.949} & 0.142 \\
CoMusion (ECCV 2024) & 44.8 / 65.7 & -1.28 & \textbf{0.950} & \underline{0.131} & 152.7 / 168.8 & 22.95 & \underline{0.951} & 0.547 & 32.4 / 59.4 & -1.31 & 0.948 & \underline{0.110} \\
SPARD (AAAI 2026) & \textbf{44.5 / 64.5} & -1.39 & \underline{0.949} & \textbf{0.129} & 152.2 / 176.1 & 22.71 & \textbf{0.950} & 0.473 & 32.9 / 61.0 & -1.40 & \underline{0.951} & \textbf{0.107} \\
MotionMap (CVPR 2025) & 161.2 / 165.5 & 3.15 & 0.953 & 0.435 & 173.2 / 166.5 & 50.54 & 0.944 & 0.431 & 179.3 / 190.2 & 15.52 & \underline{0.951} & 0.532 \\
SLD-HMP (ECCV 2024) & 54.3 / 80.1 & 4.17 & 0.948 & 0.162 & 58.4 / 80.4 & 7.34 & 0.936 & \textbf{0.155} & 52.0 / 76.7 & 7.91 & 0.948 & 0.193 \\
\textbf{CSM + SPECTRA-CP (Mondrian-pen)} & 48.0 / 71.8 & \textbf{-2.24} & 0.948 & 0.138 & 63.0 / 86.5 & \underline{-1.61} & 0.954 & \underline{0.201} & 49.3 / 94.9 & \textbf{-2.01} & 0.948 & 0.158 \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included). For Cov95(CP), best/second-best are defined by closeness to the 0.95 target.}
{\footnotesize Dataset-specific protocol-only baselines (e.g., CHICO-only SeSGCN protocol variants) are omitted to avoid redundant all-dataset rows.}
\end{table}


==> tables/overview_csm_avg_rank.tex <==
\begin{table}[t]
\centering
\caption{Mean rank (MR; $\downarrow$ better) across datasets. Ranks are computed per dataset and averaged over available datasets. $\mathrm{MR}_{\mathrm{MPJPE+NLL}}$ is the mean of MPJPE and NLL ranks (available for all models).}
\label{tab:overview_csm_rank}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.10}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & $\mathrm{MR}_{\mathrm{MPJPE}}\downarrow$ & $\mathrm{MR}_{\mathrm{NLL}}\downarrow$ & $\mathrm{MR}_{W95(\mathrm{CP})}\downarrow$ & $\mathrm{MR}_{\mathrm{MPJPE+NLL}}\downarrow$ \\
\midrule
siMLPe (base) & 7.94 & 10.89 & -- & 9.42 \\
MeanFT (siMLPe fine-tune) & \textbf{2.39} & 6.22 & -- & \underline{4.31} \\
AuxTasks (50/50) & 9.06 & 12.00 & -- & 10.53 \\
Symplectic (50/50) & 16.22 & 15.78 & -- & 16.00 \\
DeFeeNet (50/50) & 7.94 & 10.78 & -- & 9.36 \\
GSPS (50/50) & 5.94 & 8.56 & -- & 7.25 \\
HumanMAC (50/50) & 9.78 & 10.22 & -- & 10.00 \\
SeSGCN (teacher) & 13.28 & 11.78 & -- & 12.53 \\
Deep ensemble & 5.83 & 4.44 & -- & 5.14 \\
Bridge-CQR & \underline{3.17} & \underline{2.22} & -- & \textbf{2.69} \\
SkeletonDiffusion (CVPR 2025)~\citep{curreli2025nonisotropic} & 15.11 & 13.78 & 7.44 & 14.44 \\
BeLFusion (ICCV 2023)~\citep{barquero2023belfusion} & 9.33 & 8.22 & 4.44 & 8.78 \\
TransFusion (RA-L 2024)~\citep{tian2024transfusion} & 12.44 & 10.11 & 3.67 & 11.28 \\
CoMusion (ECCV 2024)~\citep{sun2024comusion} & 6.11 & 6.67 & \underline{2.72} & 6.39 \\
SPARD (AAAI 2026)~\citep{zhang2026spard} & 7.11 & 6.78 & \textbf{2.61} & 6.94 \\
MotionMap (CVPR 2025)~\citep{hosseininejad2025motionmap} & 16.44 & 16.22 & 7.00 & 16.33 \\
SLD-HMP (ECCV 2024)~\citep{xu2024learning} & 13.22 & 15.22 & 4.78 & 14.22 \\
\textbf{CSM + SPECTRA-CP (Mondrian-pen)} & 9.67 & \textbf{1.11} & 3.33 & 5.39 \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included).}
\end{table}


==> tables/overview_gmrf_all_datasets.tex <==
\begin{table}[t]
\centering
\caption{Baselines vs. GMRF (structured Gaussian) across datasets (H=25). Bold marks the best MPJPE/NLL/W95(CP) per dataset among the shown methods (ties included); for Cov95(CP), bold marks the value closest to the 0.95 target. Cov95(CP)/W95(CP) are split-conformal calibrated 95\% marginal tubes (coverage/width averaged over coordinates). (Trajectory-level density-set metrics are reported separately.)}
\label{tab:overview_gmrf_all}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l *{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{AMASS} & \multicolumn{4}{c}{LaFAN1} & \multicolumn{4}{c}{LaFAN1-HF} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 0.0954 & 13.55 & -- & -- & 0.5453 & 319.27 & -- & -- & 0.4046 & 172.36 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{0.0593} & 3.16 & -- & -- & \underline{0.5358} & 303.33 & -- & -- & \textbf{0.3093} & 99.80 & -- & -- \\
AuxTasks (50/50) & 0.0949 & 12.39 & -- & -- & 0.5827 & 353.83 & -- & -- & 0.4299 & 184.26 & -- & -- \\
Symplectic (50/50) & 0.1424 & 39.70 & -- & -- & 1.4504 & 3203.83 & -- & -- & 0.4756 & 280.68 & -- & -- \\
DeFeeNet (50/50) & 0.0909 & 12.15 & -- & -- & 0.5666 & 341.82 & -- & -- & 0.3992 & 169.44 & -- & -- \\
GSPS (50/50) & 0.0894 & 11.30 & -- & -- & 0.5408 & 282.97 & -- & -- & 0.3833 & 148.57 & -- & -- \\
HumanMAC (50/50) & 0.0722 & 4.34 & -- & -- & 0.5564 & 290.09 & -- & -- & 0.4477 & 166.64 & -- & -- \\
SeSGCN (teacher) & 0.1029 & 9.48 & -- & -- & 0.5872 & 314.76 & -- & -- & 0.4061 & 138.80 & -- & -- \\
Deep ensemble & 0.0869 & 3.27 & -- & -- & 0.5388 & \underline{43.45} & -- & -- & 0.3894 & 80.18 & -- & -- \\
Bridge-CQR & \textbf{0.0588} & \underline{0.10} & -- & -- & \underline{0.5358} & 139.07 & -- & -- & \underline{0.3103} & \underline{45.42} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 0.0971 & 9.02 & \textbf{0.950} & 0.334 & 0.6028 & 280.23 & \underline{0.951} & 4.209 & 1.8071 & 3357.02 & 0.959 & 32.988 \\
BeLFusion (ICCV 2023) & 0.0792 & 3.84 & 0.952 & 0.235 & 0.5618 & 251.70 & 0.952 & 1.894 & 1.0006 & 520.35 & 0.961 & 3.049 \\
TransFusion (RA-L 2024) & 0.0790 & 3.76 & \underline{0.951} & 0.198 & 0.6496 & 324.90 & \textbf{0.950} & 1.847 & 1.4215 & 1222.72 & 0.956 & 3.015 \\
CoMusion (ECCV 2024) & 0.0617 & 1.49 & 0.952 & \textbf{0.174} & \textbf{0.5268} & 219.66 & \underline{0.949} & \textbf{1.590} & 0.3604 & 92.62 & \textbf{0.950} & 1.242 \\
SPARD (AAAI 2026) & 0.0638 & 1.51 & 0.953 & \underline{0.175} & 0.5682 & 292.27 & 0.955 & \underline{1.759} & 0.3677 & 105.70 & 0.954 & \underline{1.078} \\
MotionMap (CVPR 2025) & 0.2038 & 16.42 & \underline{0.949} & 0.536 & 0.7463 & 351.70 & \textbf{0.950} & 2.006 & 1.4691 & 470.72 & 0.953 & 4.645 \\
SLD-HMP (ECCV 2024) & 0.1120 & 22.45 & \underline{0.949} & 0.308 & 0.6091 & 491.37 & 0.955 & 1.936 & 0.4801 & 401.14 & 0.952 & 1.347 \\
GMRF (structured Gaussian) & \underline{0.0593} & \textbf{-1.97} & \underline{0.951} & 0.233 & \underline{0.5358} & \textbf{-1.73} & \underline{0.951} & 2.091 & \underline{0.3103} & \textbf{-1.45} & \underline{0.951} & \textbf{1.004} \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CMU-MoCap} & \multicolumn{4}{c}{Human3.6M} & \multicolumn{4}{c}{3DPW} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 2.6560 & 8726.23 & -- & -- & 0.1012 & 12.84 & -- & -- & 0.0709 & 5.08 & -- & -- \\
MeanFT (siMLPe fine-tune) & 2.6709 & 8820.46 & -- & -- & \underline{0.0720} & 5.24 & -- & -- & \textbf{0.0572} & 1.71 & -- & -- \\
AuxTasks (50/50) & \textbf{2.5429} & 8292.99 & -- & -- & 0.0999 & 12.63 & -- & -- & 0.0745 & 5.27 & -- & -- \\
Symplectic (50/50) & 6.8024 & 54096.87 & -- & -- & 0.1070 & 13.08 & -- & -- & 0.1042 & 20.62 & -- & -- \\
DeFeeNet (50/50) & 2.6316 & 8633.05 & -- & -- & 0.0981 & 12.31 & -- & -- & 0.0701 & 4.99 & -- & -- \\
GSPS (50/50) & \underline{2.5981} & 8375.43 & -- & -- & 0.0961 & 11.04 & -- & -- & 0.0673 & 4.00 & -- & -- \\
HumanMAC (50/50) & 4.8433 & 21062.22 & -- & -- & 0.0982 & 7.83 & -- & -- & 0.0707 & 2.68 & -- & -- \\
SeSGCN (teacher) & 4.9092 & 20996.24 & -- & -- & 0.1119 & 9.85 & -- & -- & 0.0952 & 5.32 & -- & -- \\
Deep ensemble & 2.6659 & \underline{1786.43} & -- & -- & \textbf{0.0717} & \underline{1.72} & -- & -- & \underline{0.0577} & 0.79 & -- & -- \\
Bridge-CQR & 2.7455 & 4185.33 & -- & -- & 0.0843 & 2.25 & -- & -- & 0.0581 & \underline{-0.50} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 8.0957 & 49441.83 & \textbf{0.950} & 381.727 & 0.1242 & 13.58 & 0.947 & 0.406 & 0.0822 & 4.91 & \underline{0.948} & 0.256 \\
BeLFusion (ICCV 2023) & 3.6186 & 12261.03 & 0.954 & 14.329 & 0.1055 & 6.22 & \underline{0.948} & 0.316 & 0.0771 & 2.13 & \textbf{0.949} & 0.207 \\
TransFusion (RA-L 2024) & 8.0839 & 44901.52 & 0.952 & 25.699 & 0.1060 & 7.18 & \underline{0.948} & 0.295 & 0.0787 & 2.72 & 0.945 & \underline{0.187} \\
CoMusion (ECCV 2024) & 8.6798 & 54190.65 & 0.953 & 24.961 & 0.0944 & 4.49 & 0.945 & 0.287 & 0.0690 & 1.19 & 0.945 & \textbf{0.174} \\
SPARD (AAAI 2026) & 5.5562 & 25823.22 & 0.952 & 37.934 & 0.0928 & 4.24 & 0.947 & \textbf{0.250} & 0.0703 & 1.25 & 0.946 & \textbf{0.174} \\
MotionMap (CVPR 2025) & 5.3103 & 21490.65 & \underline{0.951} & 18.384 & 0.2504 & 29.09 & \textbf{0.951} & 0.718 & 0.1841 & 9.58 & \underline{0.948} & 0.476 \\
SLD-HMP (ECCV 2024) & 2.7547 & 16866.43 & \underline{0.951} & \underline{11.966} & 0.1170 & 26.15 & 0.947 & 0.368 & 0.0846 & 15.79 & \underline{0.948} & 0.235 \\
GMRF (structured Gaussian) & 2.7454 & \textbf{1.57} & \underline{0.949} & \textbf{8.917} & 0.0721 & \textbf{-1.79} & 0.945 & \underline{0.257} & 0.0580 & \textbf{-2.00} & \textbf{0.949} & 0.213 \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CHICO} & \multicolumn{4}{c}{HA4M} & \multicolumn{4}{c}{AnDy-onePerson} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 43.2 / 75.2 & 0.66 & -- & -- & \underline{46.1 / 57.0} & -1.08 & -- & -- & 28.0 / 70.3 & 2.00 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{42.7 / 64.8} & -0.35 & -- & -- & 53.6 / 57.7 & -1.00 & -- & -- & \underline{27.4 / 55.7} & -0.27 & -- & -- \\
AuxTasks (50/50) & 44.6 / 77.7 & 0.88 & -- & -- & 91.5 / 70.6 & 0.30 & -- & -- & 32.5 / 70.7 & 2.22 & -- & -- \\
Symplectic (50/50) & 46.6 / 91.2 & 0.77 & -- & -- & 79.5 / 364.9 & 24.42 & -- & -- & 30.2 / 105.5 & 2.62 & -- & -- \\
DeFeeNet (50/50) & 42.7 / 75.2 & 0.69 & -- & -- & 93.5 / 77.2 & 3.11 & -- & -- & 26.1 / 72.6 & 1.75 & -- & -- \\
GSPS (50/50) & 42.1 / 77.8 & 0.57 & -- & -- & \textbf{48.1 / 54.4} & -0.98 & -- & -- & 27.5 / 69.3 & 1.47 & -- & -- \\
HumanMAC (50/50) & 52.0 / 70.7 & 0.27 & -- & -- & 189.5 / 196.7 & 35.25 & -- & -- & 55.7 / 80.0 & 1.98 & -- & -- \\
SeSGCN (teacher) & 66.2 / 77.7 & 1.43 & -- & -- & 150.9 / 171.5 & 21.59 & -- & -- & 55.7 / 81.3 & 2.05 & -- & -- \\
Deep ensemble & 41.3 / 78.3 & -0.21 & -- & -- & 121.1 / 67.6 & -0.56 & -- & -- & 25.4 / 69.3 & 0.53 & -- & -- \\
Bridge-CQR & 42.7 / 65.0 & \underline{-1.46} & -- & -- & 42.0 / 76.7 & \textbf{-1.73} & -- & -- & \textbf{27.0 / 55.0} & \underline{-1.46} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 57.7 / 76.8 & 1.41 & 0.952 & 0.214 & 196.7 / 189.9 & 29.06 & 0.958 & 0.778 & 63.3 / 89.7 & 4.60 & \underline{0.949} & 0.265 \\
BeLFusion (ICCV 2023) & 48.4 / 69.7 & -1.04 & \underline{0.949} & 0.150 & 144.4 / 141.6 & 8.99 & \underline{0.951} & 0.344 & 38.7 / 68.5 & -0.14 & \textbf{0.950} & 0.150 \\
TransFusion (RA-L 2024) & 48.6 / 66.4 & -0.81 & \underline{0.949} & 0.133 & 145.5 / 170.8 & 5.43 & 0.944 & \underline{0.296} & 54.7 / 82.1 & 0.07 & \underline{0.949} & 0.142 \\
CoMusion (ECCV 2024) & 44.8 / 65.7 & -1.28 & \textbf{0.950} & \underline{0.131} & 152.7 / 168.8 & 22.95 & \underline{0.951} & 0.547 & 32.4 / 59.4 & -1.31 & 0.948 & \underline{0.110} \\
SPARD (AAAI 2026) & \textbf{44.5 / 64.5} & -1.39 & \underline{0.949} & \textbf{0.129} & 152.2 / 176.1 & 22.71 & \textbf{0.950} & 0.473 & 32.9 / 61.0 & -1.40 & \underline{0.951} & \textbf{0.107} \\
MotionMap (CVPR 2025) & 161.2 / 165.5 & 3.15 & 0.953 & 0.435 & 173.2 / 166.5 & 50.54 & 0.944 & 0.431 & 179.3 / 190.2 & 15.52 & \underline{0.951} & 0.532 \\
SLD-HMP (ECCV 2024) & 54.3 / 80.1 & 4.17 & 0.948 & 0.162 & 58.4 / 80.4 & 7.34 & 0.936 & \textbf{0.155} & 52.0 / 76.7 & 7.91 & 0.948 & 0.193 \\
GMRF (structured Gaussian) & \underline{42.7 / 64.8} & \textbf{-2.14} & 0.947 & 0.156 & 103.5 / 193.9 & \underline{-1.14} & 0.946 & 0.396 & \underline{27.4 / 55.7} & \textbf{-2.21} & \underline{0.951} & 0.152 \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included). For Cov95(CP), best/second-best are defined by closeness to the 0.95 target.}
{\footnotesize Dataset-specific protocol-only baselines (e.g., CHICO-only SeSGCN protocol variants) are omitted to avoid redundant all-dataset rows.}
\end{table}


==> tables/overview_gmrf_avg_rank.tex <==
\begin{table}[t]
\centering
\caption{Mean rank (MR; $\downarrow$ better) across datasets. Ranks are computed per dataset and averaged over available datasets. $\mathrm{MR}_{\mathrm{MPJPE+NLL}}$ is the mean of MPJPE and NLL ranks (available for all models).}
\label{tab:overview_gmrf_rank}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.10}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & $\mathrm{MR}_{\mathrm{MPJPE}}\downarrow$ & $\mathrm{MR}_{\mathrm{NLL}}\downarrow$ & $\mathrm{MR}_{W95(\mathrm{CP})}\downarrow$ & $\mathrm{MR}_{\mathrm{MPJPE+NLL}}\downarrow$ \\
\midrule
siMLPe (base) & 8.28 & 10.89 & -- & 9.58 \\
MeanFT (siMLPe fine-tune) & \textbf{2.61} & 6.22 & -- & 4.42 \\
AuxTasks (50/50) & 9.39 & 12.00 & -- & 10.69 \\
Symplectic (50/50) & 16.22 & 15.78 & -- & 16.00 \\
DeFeeNet (50/50) & 8.28 & 10.78 & -- & 9.53 \\
GSPS (50/50) & 6.50 & 8.56 & -- & 7.53 \\
HumanMAC (50/50) & 10.33 & 10.22 & -- & 10.28 \\
SeSGCN (teacher) & 13.39 & 11.78 & -- & 12.58 \\
Deep ensemble & 6.17 & 4.44 & -- & 5.31 \\
Bridge-CQR & \underline{3.72} & \underline{2.22} & -- & \underline{2.97} \\
SkeletonDiffusion (CVPR 2025)~\citep{curreli2025nonisotropic} & 15.11 & 13.78 & 7.44 & 14.44 \\
BeLFusion (ICCV 2023)~\citep{barquero2023belfusion} & 9.78 & 8.22 & 4.22 & 9.00 \\
TransFusion (RA-L 2024)~\citep{tian2024transfusion} & 12.67 & 10.11 & 3.56 & 11.39 \\
CoMusion (ECCV 2024)~\citep{sun2024comusion} & 6.56 & 6.67 & \underline{2.83} & 6.61 \\
SPARD (AAAI 2026)~\citep{zhang2026spard} & 7.56 & 6.78 & \textbf{2.61} & 7.17 \\
MotionMap (CVPR 2025)~\citep{hosseininejad2025motionmap} & 16.33 & 16.22 & 6.89 & 16.28 \\
SLD-HMP (ECCV 2024)~\citep{xu2024learning} & 13.44 & 15.22 & 4.67 & 14.33 \\
GMRF (structured Gaussian) & 4.67 & \textbf{1.11} & 3.78 & \textbf{2.89} \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included).}
\end{table}


==> tables/overview_matrixnormal_all_datasets.tex <==
\begin{table}[t]
\centering
\caption{Baselines vs. MatrixNormal (freeze-mean) across datasets (H=25). Bold marks the best MPJPE/NLL/W95(CP) per dataset among the shown methods (ties included); for Cov95(CP), bold marks the value closest to the 0.95 target. Cov95(CP)/W95(CP) are split-conformal calibrated 95\% marginal tubes (coverage/width averaged over coordinates). (Trajectory-level density-set metrics are reported separately.)}
\label{tab:overview_mn_all}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l *{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{AMASS} & \multicolumn{4}{c}{LaFAN1} & \multicolumn{4}{c}{LaFAN1-HF} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 0.0954 & 13.55 & -- & -- & 0.5453 & 319.27 & -- & -- & 0.4046 & 172.36 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{0.0593} & 3.16 & -- & -- & \underline{0.5358} & 303.33 & -- & -- & \textbf{0.3093} & 99.80 & -- & -- \\
AuxTasks (50/50) & 0.0949 & 12.39 & -- & -- & 0.5827 & 353.83 & -- & -- & 0.4299 & 184.26 & -- & -- \\
Symplectic (50/50) & 0.1424 & 39.70 & -- & -- & 1.4504 & 3203.83 & -- & -- & 0.4756 & 280.68 & -- & -- \\
DeFeeNet (50/50) & 0.0909 & 12.15 & -- & -- & 0.5666 & 341.82 & -- & -- & 0.3992 & 169.44 & -- & -- \\
GSPS (50/50) & 0.0894 & 11.30 & -- & -- & 0.5408 & 282.97 & -- & -- & 0.3833 & 148.57 & -- & -- \\
HumanMAC (50/50) & 0.0722 & 4.34 & -- & -- & 0.5564 & 290.09 & -- & -- & 0.4477 & 166.64 & -- & -- \\
SeSGCN (teacher) & 0.1029 & 9.48 & -- & -- & 0.5872 & 314.76 & -- & -- & 0.4061 & 138.80 & -- & -- \\
Deep ensemble & 0.0869 & 3.27 & -- & -- & 0.5388 & \underline{43.45} & -- & -- & 0.3894 & 80.18 & -- & -- \\
Bridge-CQR & \textbf{0.0588} & \underline{0.10} & -- & -- & \underline{0.5358} & 139.07 & -- & -- & \underline{0.3103} & \underline{45.42} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 0.0971 & 9.02 & \textbf{0.950} & 0.334 & 0.6028 & 280.23 & \underline{0.951} & 4.209 & 1.8071 & 3357.02 & 0.959 & 32.988 \\
BeLFusion (ICCV 2023) & 0.0792 & 3.84 & 0.952 & 0.235 & 0.5618 & 251.70 & 0.952 & 1.894 & 1.0006 & 520.35 & 0.961 & 3.049 \\
TransFusion (RA-L 2024) & 0.0790 & 3.76 & \underline{0.951} & 0.198 & 0.6496 & 324.90 & \textbf{0.950} & 1.847 & 1.4215 & 1222.72 & 0.956 & 3.015 \\
CoMusion (ECCV 2024) & 0.0617 & 1.49 & 0.952 & \textbf{0.174} & \textbf{0.5268} & 219.66 & \underline{0.949} & \textbf{1.590} & 0.3604 & 92.62 & \textbf{0.950} & 1.242 \\
SPARD (AAAI 2026) & 0.0638 & 1.51 & 0.953 & \underline{0.175} & 0.5682 & 292.27 & 0.955 & 1.759 & 0.3677 & 105.70 & 0.954 & \underline{1.078} \\
MotionMap (CVPR 2025) & 0.2038 & 16.42 & \underline{0.949} & 0.536 & 0.7463 & 351.70 & \textbf{0.950} & 2.006 & 1.4691 & 470.72 & 0.953 & 4.645 \\
SLD-HMP (ECCV 2024) & 0.1120 & 22.45 & \underline{0.949} & 0.308 & 0.6091 & 491.37 & 0.955 & 1.936 & 0.4801 & 401.14 & 0.952 & 1.347 \\
\textbf{MatrixNormal (freeze-mean)} & \underline{0.0593} & \textbf{-2.67} & \underline{0.951} & 0.184 & \underline{0.5358} & \textbf{1.69} & 0.952 & \underline{1.623} & \underline{0.3103} & \textbf{6.10} & \underline{0.951} & \textbf{0.994} \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CMU-MoCap} & \multicolumn{4}{c}{Human3.6M} & \multicolumn{4}{c}{3DPW} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 2.6560 & 8726.23 & -- & -- & 0.1012 & 12.84 & -- & -- & 0.0709 & 5.08 & -- & -- \\
MeanFT (siMLPe fine-tune) & 2.6709 & 8820.46 & -- & -- & \underline{0.0720} & 5.24 & -- & -- & \textbf{0.0572} & 1.71 & -- & -- \\
AuxTasks (50/50) & \textbf{2.5429} & 8292.99 & -- & -- & 0.0999 & 12.63 & -- & -- & 0.0745 & 5.27 & -- & -- \\
Symplectic (50/50) & 6.8024 & 54096.87 & -- & -- & 0.1070 & 13.08 & -- & -- & 0.1042 & 20.62 & -- & -- \\
DeFeeNet (50/50) & 2.6316 & 8633.05 & -- & -- & 0.0981 & 12.31 & -- & -- & 0.0701 & 4.99 & -- & -- \\
GSPS (50/50) & \underline{2.5981} & 8375.43 & -- & -- & 0.0961 & 11.04 & -- & -- & 0.0673 & 4.00 & -- & -- \\
HumanMAC (50/50) & 4.8433 & 21062.22 & -- & -- & 0.0982 & 7.83 & -- & -- & 0.0707 & 2.68 & -- & -- \\
SeSGCN (teacher) & 4.9092 & 20996.24 & -- & -- & 0.1119 & 9.85 & -- & -- & 0.0952 & 5.32 & -- & -- \\
Deep ensemble & 2.6659 & \underline{1786.43} & -- & -- & \textbf{0.0717} & \underline{1.72} & -- & -- & \underline{0.0577} & 0.79 & -- & -- \\
Bridge-CQR & 2.7455 & 4185.33 & -- & -- & 0.0843 & 2.25 & -- & -- & 0.0581 & \underline{-0.50} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 8.0957 & 49441.83 & \textbf{0.950} & 381.727 & 0.1242 & 13.58 & 0.947 & 0.406 & 0.0822 & 4.91 & \underline{0.948} & 0.256 \\
BeLFusion (ICCV 2023) & 3.6186 & 12261.03 & 0.954 & 14.329 & 0.1055 & 6.22 & \underline{0.948} & 0.316 & 0.0771 & 2.13 & \textbf{0.949} & 0.207 \\
TransFusion (RA-L 2024) & 8.0839 & 44901.52 & 0.952 & 25.699 & 0.1060 & 7.18 & \underline{0.948} & 0.295 & 0.0787 & 2.72 & 0.945 & 0.187 \\
CoMusion (ECCV 2024) & 8.6798 & 54190.65 & 0.953 & 24.961 & 0.0944 & 4.49 & 0.945 & 0.287 & 0.0690 & 1.19 & 0.945 & \underline{0.174} \\
SPARD (AAAI 2026) & 5.5562 & 25823.22 & 0.952 & 37.934 & 0.0928 & 4.24 & 0.947 & \textbf{0.250} & 0.0703 & 1.25 & 0.946 & \underline{0.174} \\
MotionMap (CVPR 2025) & 5.3103 & 21490.65 & \underline{0.951} & 18.384 & 0.2504 & 29.09 & \textbf{0.951} & 0.718 & 0.1841 & 9.58 & \underline{0.948} & 0.476 \\
SLD-HMP (ECCV 2024) & 2.7547 & 16866.43 & \underline{0.951} & \underline{11.966} & 0.1170 & 26.15 & 0.947 & 0.368 & 0.0846 & 15.79 & \underline{0.948} & 0.235 \\
\textbf{MatrixNormal (freeze-mean)} & 2.7454 & \textbf{135.89} & \underline{0.951} & \textbf{9.339} & 0.0721 & \textbf{-1.26} & 0.945 & \underline{0.253} & 0.0580 & \textbf{-1.89} & 0.946 & \textbf{0.173} \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CHICO} & \multicolumn{4}{c}{HA4M} & \multicolumn{4}{c}{AnDy-onePerson} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 43.2 / 75.2 & 0.66 & -- & -- & \underline{46.1 / 57.0} & \underline{-1.08} & -- & -- & 28.0 / 70.3 & 2.00 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{42.7 / 64.8} & -0.35 & -- & -- & 53.6 / 57.7 & -1.00 & -- & -- & \underline{27.4 / 55.7} & -0.27 & -- & -- \\
AuxTasks (50/50) & 44.6 / 77.7 & 0.88 & -- & -- & 91.5 / 70.6 & 0.30 & -- & -- & 32.5 / 70.7 & 2.22 & -- & -- \\
Symplectic (50/50) & 46.6 / 91.2 & 0.77 & -- & -- & 79.5 / 364.9 & 24.42 & -- & -- & 30.2 / 105.5 & 2.62 & -- & -- \\
DeFeeNet (50/50) & 42.7 / 75.2 & 0.69 & -- & -- & 93.5 / 77.2 & 3.11 & -- & -- & 26.1 / 72.6 & 1.75 & -- & -- \\
GSPS (50/50) & 42.1 / 77.8 & 0.57 & -- & -- & \textbf{48.1 / 54.4} & -0.98 & -- & -- & 27.5 / 69.3 & 1.47 & -- & -- \\
HumanMAC (50/50) & 52.0 / 70.7 & 0.27 & -- & -- & 189.5 / 196.7 & 35.25 & -- & -- & 55.7 / 80.0 & 1.98 & -- & -- \\
SeSGCN (teacher) & 66.2 / 77.7 & 1.43 & -- & -- & 150.9 / 171.5 & 21.59 & -- & -- & 55.7 / 81.3 & 2.05 & -- & -- \\
Deep ensemble & 41.3 / 78.3 & -0.21 & -- & -- & 121.1 / 67.6 & -0.56 & -- & -- & 25.4 / 69.3 & 0.53 & -- & -- \\
Bridge-CQR & 42.7 / 65.0 & \underline{-1.46} & -- & -- & 42.0 / 76.7 & \textbf{-1.73} & -- & -- & \textbf{27.0 / 55.0} & \underline{-1.46} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 57.7 / 76.8 & 1.41 & 0.952 & 0.214 & 196.7 / 189.9 & 29.06 & 0.958 & 0.778 & 63.3 / 89.7 & 4.60 & \underline{0.949} & 0.265 \\
BeLFusion (ICCV 2023) & 48.4 / 69.7 & -1.04 & \underline{0.949} & 0.150 & 144.4 / 141.6 & 8.99 & \underline{0.951} & 0.344 & 38.7 / 68.5 & -0.14 & \textbf{0.950} & 0.150 \\
TransFusion (RA-L 2024) & 48.6 / 66.4 & -0.81 & \underline{0.949} & 0.133 & 145.5 / 170.8 & 5.43 & 0.944 & \underline{0.296} & 54.7 / 82.1 & 0.07 & \underline{0.949} & 0.142 \\
CoMusion (ECCV 2024) & 44.8 / 65.7 & -1.28 & \textbf{0.950} & \underline{0.131} & 152.7 / 168.8 & 22.95 & \underline{0.951} & 0.547 & 32.4 / 59.4 & -1.31 & 0.948 & \underline{0.110} \\
SPARD (AAAI 2026) & \textbf{44.5 / 64.5} & -1.39 & \underline{0.949} & \textbf{0.129} & 152.2 / 176.1 & 22.71 & \textbf{0.950} & 0.473 & 32.9 / 61.0 & -1.40 & \underline{0.951} & \textbf{0.107} \\
MotionMap (CVPR 2025) & 161.2 / 165.5 & 3.15 & 0.953 & 0.435 & 173.2 / 166.5 & 50.54 & 0.944 & 0.431 & 179.3 / 190.2 & 15.52 & \underline{0.951} & 0.532 \\
SLD-HMP (ECCV 2024) & 54.3 / 80.1 & 4.17 & 0.948 & 0.162 & 58.4 / 80.4 & 7.34 & 0.936 & \textbf{0.155} & 52.0 / 76.7 & 7.91 & 0.948 & 0.193 \\
\textbf{MatrixNormal (freeze-mean)} & \underline{42.7 / 64.8} & \textbf{-1.68} & 0.947 & 0.154 & 103.5 / 193.9 & -0.61 & 0.944 & 0.305 & \underline{27.4 / 55.7} & \textbf{-1.98} & \underline{0.951} & 0.138 \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included). For Cov95(CP), best/second-best are defined by closeness to the 0.95 target.}
{\footnotesize Dataset-specific protocol-only baselines (e.g., CHICO-only SeSGCN protocol variants) are omitted to avoid redundant all-dataset rows.}
\end{table}


==> tables/overview_matrixnormal_avg_rank.tex <==
\begin{table}[t]
\centering
\caption{Mean rank (MR; $\downarrow$ better) across datasets. Ranks are computed per dataset and averaged over available datasets. $\mathrm{MR}_{\mathrm{MPJPE+NLL}}$ is the mean of MPJPE and NLL ranks (available for all models).}
\label{tab:overview_mn_rank}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.10}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & $\mathrm{MR}_{\mathrm{MPJPE}}\downarrow$ & $\mathrm{MR}_{\mathrm{NLL}}\downarrow$ & $\mathrm{MR}_{W95(\mathrm{CP})}\downarrow$ & $\mathrm{MR}_{\mathrm{MPJPE+NLL}}\downarrow$ \\
\midrule
siMLPe (base) & 8.28 & 10.78 & -- & 9.53 \\
MeanFT (siMLPe fine-tune) & \textbf{2.61} & 6.11 & -- & 4.36 \\
AuxTasks (50/50) & 9.39 & 12.00 & -- & 10.69 \\
Symplectic (50/50) & 16.22 & 15.78 & -- & 16.00 \\
DeFeeNet (50/50) & 8.28 & 10.78 & -- & 9.53 \\
GSPS (50/50) & 6.50 & 8.44 & -- & 7.47 \\
HumanMAC (50/50) & 10.33 & 10.22 & -- & 10.28 \\
SeSGCN (teacher) & 13.39 & 11.78 & -- & 12.58 \\
Deep ensemble & 6.17 & 4.44 & -- & 5.31 \\
Bridge-CQR & \underline{3.72} & \underline{2.22} & -- & \textbf{2.97} \\
SkeletonDiffusion (CVPR 2025)~\citep{curreli2025nonisotropic} & 15.11 & 13.78 & 7.44 & 14.44 \\
BeLFusion (ICCV 2023)~\citep{barquero2023belfusion} & 9.78 & 8.22 & 4.67 & 9.00 \\
TransFusion (RA-L 2024)~\citep{tian2024transfusion} & 12.67 & 10.11 & 4.00 & 11.39 \\
CoMusion (ECCV 2024)~\citep{sun2024comusion} & 6.56 & 6.67 & 2.94 & 6.61 \\
SPARD (AAAI 2026)~\citep{zhang2026spard} & 7.56 & 6.78 & \underline{2.83} & 7.17 \\
MotionMap (CVPR 2025)~\citep{hosseininejad2025motionmap} & 16.33 & 16.22 & 7.00 & 16.28 \\
SLD-HMP (ECCV 2024)~\citep{xu2024learning} & 13.44 & 15.22 & 4.78 & 14.33 \\
\textbf{MatrixNormal (freeze-mean)} & 4.67 & \textbf{1.44} & \textbf{2.33} & \underline{3.06} \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included).}
\end{table}


==> tables/overview_mngraph_all_datasets.tex <==
\begin{table}[t]
\centering
\caption{Baselines vs. MatrixNormal-GraphJ (freeze-mean) across datasets (H=25). Bold marks the best MPJPE/NLL/W95(CP) per dataset among the shown methods (ties included); for Cov95(CP), bold marks the value closest to the 0.95 target. Cov95(CP)/W95(CP) are split-conformal calibrated 95\% marginal tubes (coverage/width averaged over coordinates). (Trajectory-level density-set metrics are reported separately.)}
\label{tab:overview_mngraph_all}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l *{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{AMASS} & \multicolumn{4}{c}{LaFAN1} & \multicolumn{4}{c}{LaFAN1-HF} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 0.0954 & 13.55 & -- & -- & 0.5453 & 319.27 & -- & -- & 0.4046 & 172.36 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{0.0593} & 3.16 & -- & -- & \underline{0.5358} & 303.33 & -- & -- & \textbf{0.3093} & 99.80 & -- & -- \\
AuxTasks (50/50) & 0.0949 & 12.39 & -- & -- & 0.5827 & 353.83 & -- & -- & 0.4299 & 184.26 & -- & -- \\
Symplectic (50/50) & 0.1424 & 39.70 & -- & -- & 1.4504 & 3203.83 & -- & -- & 0.4756 & 280.68 & -- & -- \\
DeFeeNet (50/50) & 0.0909 & 12.15 & -- & -- & 0.5666 & 341.82 & -- & -- & 0.3992 & 169.44 & -- & -- \\
GSPS (50/50) & 0.0894 & 11.30 & -- & -- & 0.5408 & 282.97 & -- & -- & 0.3833 & 148.57 & -- & -- \\
HumanMAC (50/50) & 0.0722 & 4.34 & -- & -- & 0.5564 & 290.09 & -- & -- & 0.4477 & 166.64 & -- & -- \\
SeSGCN (teacher) & 0.1029 & 9.48 & -- & -- & 0.5872 & 314.76 & -- & -- & 0.4061 & 138.80 & -- & -- \\
Deep ensemble & 0.0869 & 3.27 & -- & -- & 0.5388 & \underline{43.45} & -- & -- & 0.3894 & 80.18 & -- & -- \\
Bridge-CQR & \textbf{0.0588} & \underline{0.10} & -- & -- & \underline{0.5358} & 139.07 & -- & -- & \underline{0.3103} & \underline{45.42} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 0.0971 & 9.02 & \textbf{0.950} & 0.334 & 0.6028 & 280.23 & \underline{0.951} & 4.209 & 1.8071 & 3357.02 & 0.959 & 32.988 \\
BeLFusion (ICCV 2023) & 0.0792 & 3.84 & 0.952 & 0.235 & 0.5618 & 251.70 & 0.952 & 1.894 & 1.0006 & 520.35 & 0.961 & 3.049 \\
TransFusion (RA-L 2024) & 0.0790 & 3.76 & \underline{0.951} & 0.198 & 0.6496 & 324.90 & \textbf{0.950} & 1.847 & 1.4215 & 1222.72 & 0.956 & 3.015 \\
CoMusion (ECCV 2024) & 0.0617 & 1.49 & 0.952 & \textbf{0.174} & \textbf{0.5268} & 219.66 & \underline{0.949} & \textbf{1.590} & 0.3604 & 92.62 & \textbf{0.950} & 1.242 \\
SPARD (AAAI 2026) & 0.0638 & 1.51 & 0.953 & \underline{0.175} & 0.5682 & 292.27 & 0.955 & \underline{1.759} & 0.3677 & 105.70 & 0.954 & \underline{1.078} \\
MotionMap (CVPR 2025) & 0.2038 & 16.42 & \underline{0.949} & 0.536 & 0.7463 & 351.70 & \textbf{0.950} & 2.006 & 1.4691 & 470.72 & 0.953 & 4.645 \\
SLD-HMP (ECCV 2024) & 0.1120 & 22.45 & \underline{0.949} & 0.308 & 0.6091 & 491.37 & 0.955 & 1.936 & 0.4801 & 401.14 & 0.952 & 1.347 \\
\textbf{MatrixNormal-GraphJ (freeze-mean)} & \underline{0.0593} & \textbf{-2.37} & \underline{0.951} & 0.220 & \underline{0.5358} & \textbf{-0.83} & \underline{0.951} & 2.089 & \underline{0.3103} & \textbf{-0.05} & \underline{0.951} & \textbf{1.012} \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CMU-MoCap} & \multicolumn{4}{c}{Human3.6M} & \multicolumn{4}{c}{3DPW} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 2.6560 & 8726.23 & -- & -- & 0.1012 & 12.84 & -- & -- & 0.0709 & 5.08 & -- & -- \\
MeanFT (siMLPe fine-tune) & 2.6709 & 8820.46 & -- & -- & \underline{0.0720} & 5.24 & -- & -- & \textbf{0.0572} & 1.71 & -- & -- \\
AuxTasks (50/50) & \textbf{2.5429} & 8292.99 & -- & -- & 0.0999 & 12.63 & -- & -- & 0.0745 & 5.27 & -- & -- \\
Symplectic (50/50) & 6.8024 & 54096.87 & -- & -- & 0.1070 & 13.08 & -- & -- & 0.1042 & 20.62 & -- & -- \\
DeFeeNet (50/50) & 2.6316 & 8633.05 & -- & -- & 0.0981 & 12.31 & -- & -- & 0.0701 & 4.99 & -- & -- \\
GSPS (50/50) & \underline{2.5981} & 8375.43 & -- & -- & 0.0961 & 11.04 & -- & -- & 0.0673 & 4.00 & -- & -- \\
HumanMAC (50/50) & 4.8433 & 21062.22 & -- & -- & 0.0982 & 7.83 & -- & -- & 0.0707 & 2.68 & -- & -- \\
SeSGCN (teacher) & 4.9092 & 20996.24 & -- & -- & 0.1119 & 9.85 & -- & -- & 0.0952 & 5.32 & -- & -- \\
Deep ensemble & 2.6659 & \underline{1786.43} & -- & -- & \textbf{0.0717} & \underline{1.72} & -- & -- & \underline{0.0577} & 0.79 & -- & -- \\
Bridge-CQR & 2.7455 & 4185.33 & -- & -- & 0.0843 & 2.25 & -- & -- & 0.0581 & \underline{-0.50} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 8.0957 & 49441.83 & \textbf{0.950} & 381.727 & 0.1242 & 13.58 & 0.947 & 0.406 & 0.0822 & 4.91 & \underline{0.948} & 0.256 \\
BeLFusion (ICCV 2023) & 3.6186 & 12261.03 & 0.954 & 14.329 & 0.1055 & 6.22 & \underline{0.948} & 0.316 & 0.0771 & 2.13 & \textbf{0.949} & 0.207 \\
TransFusion (RA-L 2024) & 8.0839 & 44901.52 & 0.952 & 25.699 & 0.1060 & 7.18 & \underline{0.948} & 0.295 & 0.0787 & 2.72 & 0.945 & \underline{0.187} \\
CoMusion (ECCV 2024) & 8.6798 & 54190.65 & 0.953 & 24.961 & 0.0944 & 4.49 & 0.945 & 0.287 & 0.0690 & 1.19 & 0.945 & \textbf{0.174} \\
SPARD (AAAI 2026) & 5.5562 & 25823.22 & 0.952 & 37.934 & 0.0928 & 4.24 & 0.947 & \textbf{0.250} & 0.0703 & 1.25 & 0.946 & \textbf{0.174} \\
MotionMap (CVPR 2025) & 5.3103 & 21490.65 & \underline{0.951} & 18.384 & 0.2504 & 29.09 & \textbf{0.951} & 0.718 & 0.1841 & 9.58 & \underline{0.948} & 0.476 \\
SLD-HMP (ECCV 2024) & 2.7547 & 16866.43 & \underline{0.951} & \underline{11.966} & 0.1170 & 26.15 & 0.947 & 0.368 & 0.0846 & 15.79 & \underline{0.948} & 0.235 \\
\textbf{MatrixNormal-GraphJ (freeze-mean)} & 2.7454 & \textbf{12.94} & \textbf{0.950} & \textbf{9.225} & 0.0721 & \textbf{-1.66} & 0.945 & \underline{0.251} & 0.0580 & \textbf{-1.94} & \underline{0.948} & 0.195 \\
\addlinespace
\toprule
& \multicolumn{4}{c}{CHICO} & \multicolumn{4}{c}{HA4M} & \multicolumn{4}{c}{AnDy-onePerson} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Model & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} & {MPJPE@10/25f (mm)$\downarrow$} & {NLL$\downarrow$} & {Cov95{\tiny(CP)}} & {W95{\tiny(CP)}$\downarrow$} \\
\midrule
siMLPe (base) & 43.2 / 75.2 & 0.66 & -- & -- & \underline{46.1 / 57.0} & -1.08 & -- & -- & 28.0 / 70.3 & 2.00 & -- & -- \\
MeanFT (siMLPe fine-tune) & \underline{42.7 / 64.8} & -0.35 & -- & -- & 53.6 / 57.7 & -1.00 & -- & -- & \underline{27.4 / 55.7} & -0.27 & -- & -- \\
AuxTasks (50/50) & 44.6 / 77.7 & 0.88 & -- & -- & 91.5 / 70.6 & 0.30 & -- & -- & 32.5 / 70.7 & 2.22 & -- & -- \\
Symplectic (50/50) & 46.6 / 91.2 & 0.77 & -- & -- & 79.5 / 364.9 & 24.42 & -- & -- & 30.2 / 105.5 & 2.62 & -- & -- \\
DeFeeNet (50/50) & 42.7 / 75.2 & 0.69 & -- & -- & 93.5 / 77.2 & 3.11 & -- & -- & 26.1 / 72.6 & 1.75 & -- & -- \\
GSPS (50/50) & 42.1 / 77.8 & 0.57 & -- & -- & \textbf{48.1 / 54.4} & -0.98 & -- & -- & 27.5 / 69.3 & 1.47 & -- & -- \\
HumanMAC (50/50) & 52.0 / 70.7 & 0.27 & -- & -- & 189.5 / 196.7 & 35.25 & -- & -- & 55.7 / 80.0 & 1.98 & -- & -- \\
SeSGCN (teacher) & 66.2 / 77.7 & 1.43 & -- & -- & 150.9 / 171.5 & 21.59 & -- & -- & 55.7 / 81.3 & 2.05 & -- & -- \\
Deep ensemble & 41.3 / 78.3 & -0.21 & -- & -- & 121.1 / 67.6 & -0.56 & -- & -- & 25.4 / 69.3 & 0.53 & -- & -- \\
Bridge-CQR & 42.7 / 65.0 & \underline{-1.46} & -- & -- & 42.0 / 76.7 & \underline{-1.73} & -- & -- & \textbf{27.0 / 55.0} & \underline{-1.46} & -- & -- \\
SkeletonDiffusion (CVPR 2025) & 57.7 / 76.8 & 1.41 & 0.952 & 0.214 & 196.7 / 189.9 & 29.06 & 0.958 & 0.778 & 63.3 / 89.7 & 4.60 & \underline{0.949} & 0.265 \\
BeLFusion (ICCV 2023) & 48.4 / 69.7 & -1.04 & \underline{0.949} & 0.150 & 144.4 / 141.6 & 8.99 & \underline{0.951} & 0.344 & 38.7 / 68.5 & -0.14 & \textbf{0.950} & 0.150 \\
TransFusion (RA-L 2024) & 48.6 / 66.4 & -0.81 & \underline{0.949} & 0.133 & 145.5 / 170.8 & 5.43 & 0.944 & \underline{0.296} & 54.7 / 82.1 & 0.07 & \underline{0.949} & 0.142 \\
CoMusion (ECCV 2024) & 44.8 / 65.7 & -1.28 & \textbf{0.950} & \underline{0.131} & 152.7 / 168.8 & 22.95 & \underline{0.951} & 0.547 & 32.4 / 59.4 & -1.31 & 0.948 & \underline{0.110} \\
SPARD (AAAI 2026) & \textbf{44.5 / 64.5} & -1.39 & \underline{0.949} & \textbf{0.129} & 152.2 / 176.1 & 22.71 & \textbf{0.950} & 0.473 & 32.9 / 61.0 & -1.40 & \underline{0.951} & \textbf{0.107} \\
MotionMap (CVPR 2025) & 161.2 / 165.5 & 3.15 & 0.953 & 0.435 & 173.2 / 166.5 & 50.54 & 0.944 & 0.431 & 179.3 / 190.2 & 15.52 & \underline{0.951} & 0.532 \\
SLD-HMP (ECCV 2024) & 54.3 / 80.1 & 4.17 & 0.948 & 0.162 & 58.4 / 80.4 & 7.34 & 0.936 & \textbf{0.155} & 52.0 / 76.7 & 7.91 & 0.948 & 0.193 \\
\textbf{MatrixNormal-GraphJ (freeze-mean)} & \underline{42.7 / 64.8} & \textbf{-2.21} & 0.947 & 0.151 & 103.5 / 193.9 & \textbf{-2.25} & 0.945 & 0.354 & \underline{27.4 / 55.7} & \textbf{-3.52} & \textbf{0.950} & 0.142 \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included). For Cov95(CP), best/second-best are defined by closeness to the 0.95 target.}
{\footnotesize Dataset-specific protocol-only baselines (e.g., CHICO-only SeSGCN protocol variants) are omitted to avoid redundant all-dataset rows.}
\end{table}


==> tables/overview_mngraph_avg_rank.tex <==
\begin{table}[t]
\centering
\caption{Mean rank (MR; $\downarrow$ better) across datasets. Ranks are computed per dataset and averaged over available datasets. $\mathrm{MR}_{\mathrm{MPJPE+NLL}}$ is the mean of MPJPE and NLL ranks (available for all models).}
\label{tab:overview_mngraph_rank}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.10}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & $\mathrm{MR}_{\mathrm{MPJPE}}\downarrow$ & $\mathrm{MR}_{\mathrm{NLL}}\downarrow$ & $\mathrm{MR}_{W95(\mathrm{CP})}\downarrow$ & $\mathrm{MR}_{\mathrm{MPJPE+NLL}}\downarrow$ \\
\midrule
siMLPe (base) & 8.28 & 10.89 & -- & 9.58 \\
MeanFT (siMLPe fine-tune) & \textbf{2.61} & 6.22 & -- & 4.42 \\
AuxTasks (50/50) & 9.39 & 12.00 & -- & 10.69 \\
Symplectic (50/50) & 16.22 & 15.78 & -- & 16.00 \\
DeFeeNet (50/50) & 8.28 & 10.78 & -- & 9.53 \\
GSPS (50/50) & 6.50 & 8.56 & -- & 7.53 \\
HumanMAC (50/50) & 10.33 & 10.22 & -- & 10.28 \\
SeSGCN (teacher) & 13.39 & 11.78 & -- & 12.58 \\
Deep ensemble & 6.17 & 4.44 & -- & 5.31 \\
Bridge-CQR & \underline{3.72} & \underline{2.33} & -- & \underline{3.03} \\
SkeletonDiffusion (CVPR 2025)~\citep{curreli2025nonisotropic} & 15.11 & 13.78 & 7.44 & 14.44 \\
BeLFusion (ICCV 2023)~\citep{barquero2023belfusion} & 9.78 & 8.22 & 4.44 & 9.00 \\
TransFusion (RA-L 2024)~\citep{tian2024transfusion} & 12.67 & 10.11 & 3.61 & 11.39 \\
CoMusion (ECCV 2024)~\citep{sun2024comusion} & 6.56 & 6.67 & \underline{2.83} & 6.61 \\
SPARD (AAAI 2026)~\citep{zhang2026spard} & 7.56 & 6.78 & \textbf{2.61} & 7.17 \\
MotionMap (CVPR 2025)~\citep{hosseininejad2025motionmap} & 16.33 & 16.22 & 6.89 & 16.28 \\
SLD-HMP (ECCV 2024)~\citep{xu2024learning} & 13.44 & 15.22 & 4.67 & 14.33 \\
\textbf{MatrixNormal-GraphJ (freeze-mean)} & 4.67 & \textbf{1.00} & 3.50 & \textbf{2.83} \\
\bottomrule
\end{tabular}
}
\par\smallskip
{\footnotesize\textbf{Legend:} \textbf{bold} = best; \underline{underline} = second-best (ties included).}
\end{table}


==> tables/pw3d_conjgraph_kappa_mondrian.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
$\sqrt{\kappa}$ bin & \#Seq. & Cov90(CP) & W90(CP)$\downarrow$ & Cov90(Mondrian) & W90(Mondrian)$\downarrow$ \\
\midrule
0--20\% [1.000187,1.000500) & 215 & 0.969 & 0.122 & 0.903 & 0.065 \\
20--40\% [1.000500,1.001123) & 225 & 0.924 & 0.124 & 0.900 & 0.107 \\
40--60\% [1.001123,1.002144) & 202 & 0.880 & 0.129 & 0.885 & 0.135 \\
60--80\% [1.002144,1.003056) & 167 & 0.868 & 0.135 & 0.893 & 0.156 \\
80--100\% [1.003056,1.014073) & 215 & 0.832 & 0.138 & 0.899 & 0.191 \\
\midrule
All & 1024 & 0.896 & 0.129 & 0.896 & 0.129 \\
\bottomrule
\end{tabular}
\caption{3DPW: $\kappa$-conditioned (Mondrian) split conformal for marginal tubes. Protocol: calibrate on held-out windows (n=512), evaluate on disjoint test windows (n=1024), target $\alpha=0.1$, and form 5 calibration-set quantile bins by mean $\sqrt{\kappa_t(x)}$. The table compares unconditioned CP with Mondrian bin-wise calibration using marginal coverage (Cov90) and mean interval width (W90).}
\label{tab:pw3d_kappa_mondrian}
\end{table}


==> tables/pw3d_conjgraph_traj_set.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrr@{}}
\toprule
Set & Coverage & $\log$Vol$/d$ $\downarrow$ \\
\midrule
Marginal tube (CP) & 0.896 & -2.221 \\
Trajectory ellipsoid (Mahalanobis CP) & 0.918 & -1.637 \\
\bottomrule
\end{tabular}
\caption{3DPW: trajectory-level conformal ellipsoid from the structured hybrid covariance. Protocol: $n_{\mathrm{cal}}=512$, $n_{\mathrm{eval}}=1024$, $\alpha=0.1$. The table compares the axis-aligned CP rectangle with the conformal ellipsoid induced by the structured Mahalanobis/whitened-residual score under $\Sigma_T^{\mathrm{hyb}}\otimes\Sigma_C$; $\log$Vol$/d$ is mean log-volume per dimension (lower is tighter).}
\label{tab:pw3d_traj_set}
\end{table}


==> tables/trajectory_set_metrics_all_datasets.tex <==
% Auto-generated by scripts/paper/eval_mn_densityset_setmetrics_all_datasets.py
\begin{table}[t]
  \centering
  \caption{Trajectory-level density-set metrics across datasets (target 90\%). Cov90(Set) is empirical set membership for the full trajectory; logV/dim is the mean log-volume per dimension (a set-size proxy, up to an additive constant).}
  \label{tab:set_metrics_all_datasets}
  \scriptsize
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.10}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}lrrrrrr@{}}
    \toprule
    Dataset & $d$ & $n_{\mathrm{cal}}$ & $n_{\mathrm{eval}}$ & Cov90(Model) & Cov90(Set) & logV/dim \\
    \midrule
    AMASS & 1350 & 512 & 1024 & 0.695 & 0.903 & -1.8948 \\
    LaFAN1 & 5625 & 512 & 1024 & 0.104 & 0.878 & 0.6737 \\
    LaFAN1-HF & 900 & 512 & 1024 & 0.016 & 0.898 & 0.2623 \\
    CMU-MoCap & 2325 & 512 & 320 & 0.028 & 0.906 & 1.9439 \\
    Human3.6M & 1650 & 512 & 1024 & 0.613 & 0.911 & -0.8961 \\
    3DPW & 1350 & 512 & 1024 & 0.940 & 0.911 & -2.2656 \\
    CHICO & 1125 & 512 & 1024 & 0.943 & 0.896 & -1.4878 \\
    HA4M & 2400 & 25 & 1 & 1.000 & 1.000 & -0.8240 \\
    AnDy-onePerson & 1725 & 512 & 1024 & 0.848 & 0.882 & -1.2455 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/trajectory_set_metrics_mngraph_all_datasets.tex <==
% Auto-generated by scripts/paper/eval_mngraph_densityset_setmetrics_all_datasets.py
\begin{table}[t]
  \centering
  \caption{Trajectory-level density-set metrics for MatrixNormalGraph across datasets (target 90\%). Cov90(Set) uses density-set conformal prediction (NLL threshold) for the full trajectory; logV/dim is a mean log-volume proxy per dimension.}
  \label{tab:set_metrics_mngraph_all_datasets}
  \scriptsize
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.10}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}lrrrrrr@{}}
    \toprule
    Dataset & $d$ & $n_{\mathrm{cal}}$ & $n_{\mathrm{eval}}$ & Cov90(Model) & Cov90(Set) & logV/dim \\
    \midrule
    AMASS & 1350 & 512 & 1024 & 0.567 & 0.890 & -1.5059 \\
    LaFAN1 & 5625 & 512 & 1024 & 0.584 & 0.895 & -0.5123 \\
    LaFAN1-HF & 900 & 512 & 1024 & 0.813 & 0.900 & 0.2151 \\
    CMU-MoCap & 2325 & 512 & 320 & 0.175 & 0.897 & 1.5485 \\
    Human3.6M & 1650 & 512 & 1024 & 0.415 & 0.916 & -1.4431 \\
    3DPW & 1350 & 512 & 1024 & 0.810 & 0.909 & -2.1562 \\
    CHICO & 1125 & 512 & 1024 & 0.554 & 0.896 & -1.9011 \\
    HA4M & 2400 & 25 & 1 & 0.000 & 1.000 & -1.7856 \\
    AnDy-onePerson & 1725 & 512 & 1024 & 0.595 & 0.879 & -2.0289 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tikz/arch_csm.tex <==
% CSM + SPECTRA-CP overview diagram (TikZ).
% Compact version to fit \linewidth in single-column layout.
\begin{tikzpicture}[
  font=\footnotesize,
  node distance=4mm,
  box/.style={draw, rounded corners, align=center, inner sep=3pt, minimum height=8mm},
  arrow/.style={->, >=Latex, semithick},
  scale=0.82, transform shape,
]

% Input and backbone
\node[box] (xin) {Past motion\\$x_{1:T}$};
\node[box, right=8mm of xin] (dct) {DCT};
\node[box, right=8mm of dct] (trunk) {siMLPe\\trunk};

% Three heads (stacked vertically, offset right)
\node[box, above right=6mm and 10mm of trunk] (muhead) {$\hat\mu_k$};
\node[box, right=10mm of trunk] (pihead) {$\hat\pi_k$};
\node[box, below right=6mm and 10mm of trunk] (stdhead) {$\hat\sigma_k$};

% Mixture aggregation
\node[box, right=10mm of pihead] (mix) {Mixture\\$\sum_k \pi_k\mathcal{N}$};

% Time-domain mapping, moment matching and conformal
\node[box, right=6mm of mix] (idct) {IDCT +\\Var.\ prop.};
\node[box, right=6mm of idct] (mom) {Moment\\match};
\node[box, right=6mm of mom] (cp) {SPECTRA-CP\\$\bar\mu \pm q_t\bar\sigma$};

% Arrows
\draw[arrow] (xin) -- (dct);
\draw[arrow] (dct) -- (trunk);
\draw[arrow] (trunk) -- (muhead);
\draw[arrow] (trunk) -- (pihead);
\draw[arrow] (trunk) -- (stdhead);
\draw[arrow] (muhead) -| ([xshift=-2mm]mix.north west);
\draw[arrow] (pihead) -- (mix);
\draw[arrow] (stdhead) -| ([xshift=-2mm]mix.south west);
\draw[arrow] (mix) -- (idct);
\draw[arrow] (idct) -- (mom);
\draw[arrow] (mom) -- (cp);

% Annotations
\node[above=1mm of muhead, font=\tiny, gray] {means};
\node[above=1mm of pihead, font=\tiny, gray] {logits};
\node[below=1mm of stdhead, font=\tiny, gray] {log-std};
\node[below=2mm of cp, font=\tiny, align=center] {Calibrated\\90\% tubes};

\end{tikzpicture}


==> tikz/arch_mn_densityset.tex <==
% MatrixNormal + density-set CP overview diagram (TikZ).
% Designed to fit \linewidth in single-column layout.
\begin{tikzpicture}[
  font=\footnotesize,
  node distance=4mm,
  box/.style={draw, rounded corners, align=center, inner sep=3pt, minimum height=8mm},
  arrow/.style={->, >=Latex, semithick},
  scale=0.85, transform shape,
]

% Inputs / backbone
\node[box] (xin) {Past motion\\$x_{1:T}$};
\node[box, right=8mm of xin] (trunk) {MLP\\backbone};

% Heads
\node[box, above right=6mm and 10mm of trunk] (mean) {Mean\\$m_\phi(x)$};
\node[box, below right=6mm and 10mm of trunk] (cov) {Covariance\\$\Sigma_T(x),\Sigma_C(x)$};

% Density and score
\node[box, right=12mm of trunk] (dens) {MatrixNormal\\$p_\theta(y\mid x)$};
\node[box, right=10mm of dens] (score) {Score\\$s(x,y)=-\log p_\theta(y\mid x)$};
\node[box, right=10mm of score] (calib) {Calibrate\\$q_{1-\alpha}$};
\node[box, right=10mm of calib] (set) {Prediction set\\$\mathcal{C}_\alpha(x)=\{y:s\le q_{1-\alpha}\}$};

% Arrows
\draw[arrow] (xin) -- (trunk);
\draw[arrow] (trunk) -- (mean);
\draw[arrow] (trunk) -- (cov);
\draw[arrow] (mean) -| (dens.north west);
\draw[arrow] (cov) -| (dens.south west);
\draw[arrow] (dens) -- (score);
\draw[arrow] (score) -- (calib);
\draw[arrow] (calib) -- (set);

% Annotations
\node[below=1mm of calib, font=\tiny, gray, align=center] {split conformal\\on held-out calib set};
\node[below=1mm of set, font=\tiny, gray, align=center] {multivariate density\\level set / ellipsoid};

\end{tikzpicture}


